StyleTRF: Stylizing Tensorial Radiance Fields

Stylized view generation of scenes captured casually using a camera has received much attention recently. The geometry and appearance of the scene are typically captured as neural point sets or neural radiance fields in the previous work. An image stylization method is used to stylize the captured appearance by training its network jointly or iteratively with the structure capture network. The state-of-the-art SNeRF method trains the NeRF and stylization network in an alternating manner. These methods have high training time and require joint optimization. In this work, we present StyleTRF, a compact, quick-to-optimize strategy for stylized view generation using TensoRF. The appearance part is fine-tuned using sparse stylized priors of a few views rendered using the TensoRF representation for a few iterations. Our method thus effectively decouples style-adaption from view capture and is much faster than the previous methods. We show state-of-the-art results on several scenes used for this purpose.

==> src/sections/selfNotes.tex <==
 
 \subsection{Things to remember to write in the paper (SELF NOTES)}
 {
    \label{sub_sec:notes}
    \begin{itemize}
        \item Come up with a good name.
        \item Joint First Author - Rahul and Dhawal.
        \item Saurabh sir as author too.
        \item Original VM decomposition paper.
        \item Why does Johnson perform better than Gatys? Gatys is based on optimization of white noise image which depends on the randomness of initialization and the optimization method. Thus slightly different camera poses can produce different results. With Johnsons's approach, once the feed forward CNN is trained, the results are deterministic and due to spatial invariance of CNNs, slightly different camera poses give almost same results. In Gatys, even different initialization gives very different results.
        \item Our content loss and stylization loss is taken care of by Johnson's approach. (Which uses VGG feature losses.)
        \item Mention how MLP is not the best way to represent a radiance field which uses volumetric rendering. Rather, voxel grid lies closer since we perform volumetric renering.
        \item A user study?
        \item Do not fail to mention that we bring down the training to to 45 seconds (thanks to TensoRF + pretraining) in contrast to SNeRF's training strategy based on Gatys optimization which takes 5 days.
        \item Compare with full trained vs pretrained and point out geometric noise introduced in the full trained scenes. The geometric noise gets treated as geometry itself and is assigned a style in the full trained method (look at udnie fern).
        \item Mention that we received similar results on nerf synthetic which is 360 degrees. This indicates that if we use the inverted sphere approach presented by NeRF++, we can easily extend our method to unbounded 360-degree scenes by using two different TensoRFs for foreground and background.
        \item Maybe highlights in the image and show where we get consistency across different views. (Zoomed in the picture).
        \item Don't fail to mention that the mosaic style is a complicated style and we preserve it well enough in our consistent results. Something like, our approach works well on even complex styles like mosaic (fig 3).
        {\color{red}
        \item in case of udnie the style is more towards color palate rather on the structured patterns both StylizedNeRF, and ReREVST strugle to capture the subtle style succinctly. In case of StylizedNerF it could be due to the fact the combined radiance and density representation of Neural Network being optimized while the process of style adaption. 
        \item It can be argued that rather than stylizing geometric representation, we could have generated a series of novels views in a nearby trajectory and used the set of frames as input to Temporal stylization framworks like ReReVST, but we have observed that though temporal stylization methods maintain temporal stylization but fail to capture the style information welll. this can be seen in the Fig() \info{add an single column image for this}}
        {\color{blue}\item write about losses, add about implementation details roughly like for all real scene you upsample every k iters and max res and min resol. and speak about synthetic scenes.
        \item result
        \item fix CSS concepts
        \item pattern of Figure name is "Fig. <num>" eg: Fig.~\ref{fig:results}, tables => "Tbl. <num>" eg: Tbl.~\ref{fig:gatys_johnson}}
        \item spelling of colour to color
        \item Mention GPU.
    \end{itemize}
  }   
